Self-Edit: Fault-Aware Code Editor for Code Generation

Large language models (LLMs) have demonstrated an impressive ability to generate codes on competitive programming tasks. However, with limited sample numbers, LLMs still suffer from poor accuracy. Inspired by the process of human programming, we propose a generate-and-edit approach named Self-Edit that utilizes execution results of the generated code from LLMs to improve the code quality on the competitive programming task. We execute the generated code on the example test case provided in the question and wrap execution results into a supplementary comment. Utilizing this comment as guidance, our fault-aware code editor is employed to correct errors in the generated code. We perform extensive evaluations across two competitive programming datasets with nine different LLMs. Compared to directly generating from LLMs, our approach can improve the average of pass@1 by 89\% on APPS-dev, 31\% on APPS-test, and 48\% on HumanEval over nine popular code generation LLMs with parameter sizes ranging from 110M to 175B. Compared to other post-processing methods, our method demonstrates superior accuracy and efficiency.

==> draft_section/draft_intro.tex <==
Computer programming can be found in nearly all parts of society. Spanning entertainment, healthcare, education, and more, programming is an extraordinarily general tool with applications that are vast in scope. As computers are becoming more ubiquitous in modern life, rising demand for high quality code draws an ever-greater number of aspiring programmers to the profession. After years of study to become proﬁcient coders, human experts are are able to convert abstract specifications of diverse cognitive tasks into concrete programs.

Recently, large language models have shown their impressive capabilities for code generation on competitive problems, or named competitive programming. 
This task requires models to understand the natural language description and example input-output pairs (called "example tests") for a competitive problem, and generate an entire program to pass all hidden input-output pairs (called "hidden tests").
Competitive programming automatically can assist programmers to make programming more productive and accessible, yet so far incorporating innovations in AI has proven challenging. However, current large languange models are facing very low accuracy and pass rates for these hard programming problems. For examples, on the APPS dataset, a state-of-the-art code generation model, Codex, achieves 4\% accuracy if it is allowed to sample only one program per task (called pass@1).

To boost the performance of large language models on the competitive programming task, researchers are focusing on improve the pretraining process, such as collecting more high-quality pretrained data, increasing the amount of model parameters, improving pretrained model architectures or training objectives, \etc \zkc{need to cite}
These boosting methods have high requirements on time and computing resources, and are tough to achieve in most practical situations.
Another recent trend is to do large scale sampling of programs using a model and then filtering/ranking the programs based on the program execution on a small number of known unit tests to select one candidate solution or other neural networks. When given multiple programs obtained by sampling, these methods can re-order them in the decreasing order according to the execution behavior or the ranking scores of these programs. These post processing methods have proven to be very effective and they do not require any modifications to the pretrained model. However, a significant challenge is that these post processing methods based on samples requires large-scale generative sampling, which is expensive and time consuming. For example, AlphaCode shows that in order to filter out good answers, we need to sample at most 1M answers to each question, which costs $10^5$ TPU-seconds per problem. Even for neural-network based rerankers, it requires 100 samples per problems, which is no small burden. When the number of samples is limited, the performance of the model will drop suddenly \zkc{cite alphacode}, especially for pass@1 which is the most important metric because in the actual problem solving, we only have a small amount of trial and error opportunities.

% To alleviate the above issues, we propose a generate-and-edit framework for LLMs to generate code for competitive programming. Our approach is based on the problem-solving process of human programmers that firstly write a program based on the problem description and then debug and edit it with the execution results on the example tests. By analyzing the generated code of a large-scale pre-trained model, we observe that some of the generated solutions can be transfered to a correct solution through minor modifications. Figure \zkc{add an example} shows an example of generated code from GPT3 on APPS testset. This observation leads us to an important research problem on exploring approaches to edit for a higher quality code based on the generated code from LLMs. 
% To address the challenges mentioned above, we propose a generate-and-edit framework for large language models (LLMs) to generate code for competitive programming tasks. Our approach is inspired by the problem-solving process of human programmers, who typically write a program based on a problem description and then debug and refine it using the execution results on example tests. By analyzing the generated code of a pre-trained LLM, we have found that some of the solutions can be improved through minor modifications. Figure 1 shows an example of generated code from GPT-3 on the APPS test set. This observation has motivated us to investigate approaches to edit and improve the quality of code generated by LLMs.

% We propose a new generation framework for code generation. We view LLMs as black boxes considering that it is difficult to access large models, in most cases it can only be requested through the network. We design a fault-aware neural code editor for the outputs of large language models and then evaluate the final effect.  The fault-aware neural code editor is a decoder-only model that takes the generated code from the large language models and error message as input, and the error message is obtained by executing the generated code on the example tests, which is a part of the input natural description
% Our proposed framework for code generation is based on the use of large language models (LLMs) as black boxes. Given the difficulty of accessing and interacting with large models, we propose a fault-aware neural code editor that can process the outputs of LLMs and improve their quality. This code editor is a decoder-only model that takes the generated code and any error messages as input, and uses the error messages to refine the code. The error messages are obtained by executing the generated code on example tests, which are part of the input natural description. Through this process, our fault-aware neural code editor aims to improve the quality and accuracy of code generation using LLMs.

To address the challenges mentioned above, we propose a generate-and-edit framework for large language models (LLMs) to generate code for competitive programming tasks. Our approach is based on the problem-solving process of human programmers, who typically write a program based on a problem description and then debug and refine it using the execution results on example tests. By analyzing the generated code of a pre-trained LLM, we have found that some of the solutions can be improved through minor modifications. Figure 1 shows an example of generated code from GPT-3 on the APPS test set. This observation has motivated us to investigate approaches to edit and improve the quality of code generated by LLMs. To this end, we have developed a fault-aware neural code editor that takes the generated code and any error messages as input and uses them to refine the code. The error messages are obtained by executing the generated code on the example tests, which are part of the input natural description. Through this process, our code editor aims to improve the quality and accuracy of code generation using LLMs.

To evaluate the effectiveness of our generate-and-edit framework, we conducted experiments on a variety of programming tasks using different LLMs and settings. Our results show that our fault-aware neural code editor can significantly improve the quality of code generated by LLMs, reducing the number of errors and improving the performance on example tests. In particular, we observed that the use of error messages as additional input to the code editor was crucial for achieving these results. We also compared our approach with other methods for code generation and found that it outperforms them in terms of accuracy and efficiency. Overall, our experiments demonstrate the potential of our generate-and-edit framework for enhancing the capabilities of LLMs for code generation tasks.

In conclusion, our generate-and-edit framework for LLMs provides a promising approach for generating high-quality code for competitive programming tasks. By leveraging the power of LLMs and incorporating human-like problem-solving strategies, our framework enables LLMs to generate code that is more accurate and efficient than previously possible. Our fault-aware neural code editor, which takes the generated code and error messages as input, is key to achieving these improvements. Our experiments show that our approach outperforms other methods for code generation, and we believe it has the potential to significantly advance the field of code generation and accelerate the development of intelligent systems.

The contributions of this paper are listed as follows:
\begin{itemize}
    \item We propose a generate-and-edit framework for large language models (LLMs) to generate high-quality code for competitive programming tasks.
    \item We develop a fault-aware neural code editor that takes the generated code and error messages as input and uses them to refine the code, improving its quality and accuracy.
    \item We conduct experiments to evaluate the effectiveness of our approach, showing that it outperforms other methods for code generation in terms of accuracy and efficiency.
    \item We provide insights into the problem-solving process of human programmers and how it can be applied to LLMs for code generation tasks.
\end{itemize}
Overall, our work advances the field of code generation using LLMs and opens up new possibilities for the development of intelligent systems.

% In future work, we plan to extend and refine our generate-and-edit framework in several directions. One possible direction is to incorporate more advanced techniques for error detection and correction, such as natural language processing and machine learning. This would enable our code editor to handle a wider range of errors and provide more accurate and comprehensive feedback to the LLM. We also plan to explore ways of integrating our framework with other systems, such as code libraries and debugging tools, to further improve its capabilities and efficiency. Additionally, we will study the potential applications of our approach in other domains, such as natural language processing and artificial intelligence. Overall, our goal is to continue advancing the state of the art in code generation and provide new opportunities for research and development in this field.




% 我们证明了compared to a ﬁnetuning or pretraining baseline, the use of veriﬁers results in approximately the same performance boost as a 30x model size increase, and that veriﬁers scale signiﬁcantly better with increased data
% 同时我们的方法带来的提升不依赖于sample数量，在极少的sample num下，我们的模型可以取得很好的效果，尤其是pass@1指标

==> draft_section/draft_model.tex <==
% We now describe our generate-and-edit framework for code generation task. Figure \zkc{pipeline figure} provides an overview of the pipeline procedure. \ding{182} Firstly, our framework treat large language models as black-box to get the generated code given the natural language description.
% % \ie, we can only query them, but cannot modify the model structure and other content. 
% This is a reasonable assumption since the premise that the expertise and means to fine-tune the models is out of reach for most users. This design choice is motivated by three reasons: (a) there is a natural barrier to access these large models, and we can get only the output of the model for a given input via some interface (e.g., REST APIs), (b) these large language models constantly evolve and get better with each generation [10, 32]; treating them as blackboxes enables plug-and-play with minimal effort, and (c) finally, domain-specific improvements to large language models (e.g. for Python programming [15], general programming [11]) are rendered complementary to our efforts rather than competitive.
% \ding{183} For each generated code, we design a executor to obtain possible error messages by executing the example test. For different execution situations, we provide a supplementary comment to explain the specific execution situation.
% % For code that executes correctly, we provide a supplementary comment stating that the code passes the example test. For the code that fails to execute correctly, we extract the error message and the content of the wrong line in the python traceback as supplementary comments. 
% \ding{184} Based on natural language description, generated code and supplementary comments, we design a fault-aware editor to generate higher quality code.

==> old_section/abstract.tex <==
\begin{abstract}
Large language models (LLMs) have demonstrated an impressive ability to generate code for various programming tasks, even at the level of programming competitions. 
% Some models have demonstrated impressive capabilities to solve problems even at the level of programming competitions. 
However, with limited submission numbers, LLMs still suffer from a poor accuracy.
A recent trend is to do a large-scale sampling of programs with LLMs and then filter/rank the programs to select several candidate solutions.
% However, these approaches require a large-scale sampling before ranking, which is impractical for many users due to the high cost.
However, the large-scale sampling procedure entails high cost and is impractical for many users. 
% 表明问题的关键表述一定要想清楚怎么写的更准确
In this paper, we propose a generate-and-edit framework that utilizes execution results on the example test case to improve the quality of code generated by LLMs. Our fault-aware code editors are trained to fix the potential errors in the generated outputs with the guidance of any error messages. 
% example test case of the problem
% 这句话太长难了，而且附属的内容太多了

Our extensive evaluations on two competitive programming datasets and nine different LLMs demonstrate the effectiveness and universality. In particular, our framework can improve pass@1 by an average of 478\% on APPS-dev , 139\% on APPS-test and 124\% on HumanEval for nine popular code generation LLMs with parameter sizes ranging from 110M to 175B.
% 跟谁比说清楚，提升的base是什么
% Even for the chosen largest language model GPT3-175B, our editor model can improve pass@1 from 26.6\%  to 32.4\% on the APPS-dev benchmark.
% \lz{Improve xx\%}
% We also find that editing the code generated by PyCodeGPT (110M) produces comparable results to the GPT-J (6B) model.
In comparison to existing reranking methods, our method demonstrates both superior accuracy and efficiency, especially with a limited sample budget.
% 要不把数值放进来吧
\end{abstract}

==> old_section/compared_rerank_other.tex <==
\begin{table}[t]
% \footnotesize
    % \setlength\tabcolsep{3pt}
    % \renewcommand\arraystretch{0.8}
    \centering
    \caption{\small Full details of Pass Rate Results compared with the CodeRanker on the APPS dataset. We use \textit{GPT-Neo-125M-finetuned}, \textit{GPT-Neo-1.3B-finetune} and \textit{GPT-J-6B-finetuned} as the base model.}
\centering
\small
\begin{threeparttable}
\begin{tabular}{crcccc}
\toprule
\multicolumn{6}{l}{\textit{GPT-Neo-125M-finetuned}}                                                                          \\
% \midrule
% \midrule
\multicolumn{1}{l}{}         &              & \multicolumn{2}{c}{APPS-dev}  & \multicolumn{2}{c}{APPS-test} \\
\midrule
\multicolumn{1}{l}{}         & {\footnotesize Setting}      & @1        & @5        & @1        & @5        \\
\midrule
\multirow{2}{*}{\scriptsize \begin{tabular}[c]{@{}c@{}}Reported in\\ \cite{inala2022faultaware}\end{tabular}}     & {\tiny base model \tnote{$\dagger$}}   & 1.4           & 5.2           & 0.04          & 0.17          \\
                             & {\tiny + ranker} & 6.5             & \textbf{11.4}          & 0.1           & 0.5           \\
\midrule
\multirow{2}{*}{\scriptsize {Our results}} & {\tiny base model}   & 1.5             & 6.7          & 0.08          & 0.40          \\
                             & {\tiny + editor} & \textbf{8.5} & 10.2 & \textbf{0.22} & \textbf{0.70} \\
\midrule
\midrule

\multicolumn{6}{l}{\textit{GPT-Neo-1.3B-finetuned}}    \\
\multicolumn{1}{l}{}         &    & \multicolumn{2}{c}{APPS-dev}  & \multicolumn{2}{c}{APPS-test} \\
\midrule
\multicolumn{1}{l}{}         & {\scriptsize Setting}      & @1        & @5        & @1        & @5        \\
\midrule
\multirow{2}{*}{\scriptsize \begin{tabular}[c]{@{}c@{}}Reported in\\ \cite{inala2022faultaware}\end{tabular}}     & {\tiny base model \tnote{$\dagger$}}   & 2.6           & 9.1           & 0.14          & 0.53          \\
                             & {\tiny + ranker} & 8.0             & 15.1          & 0.3           & 1.1           \\
\midrule
\multirow{2}{*}{\scriptsize {Our results}} & {\tiny base model}  & 4.0             & 10.9          & 0.14          & 0.74          \\
                             & {\tiny + editor}& \textbf{10.5} & \textbf{18.6} & \textbf{0.68} & \textbf{1.38} \\




\midrule
\midrule
\multicolumn{6}{l}{\textit{GPT-J-6B-finetuned}}                                                                          \\
% \midrule
% \midrule
\multicolumn{1}{l}{}         &              & \multicolumn{2}{c}{APPS-dev}  & \multicolumn{2}{c}{APPS-test} \\
\midrule
\multicolumn{1}{l}{}         & {\footnotesize Setting}      & @1        & @5        & @1        & @5        \\
\midrule
\multirow{2}{*}{\scriptsize \begin{tabular}[c]{@{}c@{}}Reported in\\ \cite{inala2022faultaware}\end{tabular}}     & {\tiny base model \tnote{$\dagger$}}   & 5.1           & 15.6           & 0.5          & 1.6          \\
                             & {\tiny + ranker} & 11.0             & 21.7          & 0.8           & 2.6           \\
\midrule
\multirow{2}{*}{\scriptsize {Our results}} & {\tiny base model}   & 6.0             & 17.9          & 0.7          & 2.46          \\
                             & {\tiny + editor} & \textbf{12.0} & \textbf{27.8} & \textbf{1.4} & \textbf{3.34} \\
\bottomrule
\end{tabular}
\begin{tablenotes}
\footnotesize
     \item[$\dagger$] As CodeRanker does not release the weights of base models, we cite their results from \citea{inala2022faultaware} and reproduce finetuned base models shown in the \textit{"base model"} row below.
\end{tablenotes}
\end{threeparttable}
\vspace{-2mm}
   \label{tab:compared_rerank_other}
\end{table}

==> section/abstract_v1.tex <==
\begin{abstract}
Large language models (LLMs) have demonstrated an impressive ability to generate code for various programming tasks, even at the level of programming competitions. 
% Some models have demonstrated impressive capabilities to solve problems even at the level of programming competitions. 
However, with limited submission numbers, LLMs still suffer from a poor accuracy.
% A recent trend is to do a large-scale sampling of programs with LLMs and then filter/rank the programs to select several candidate solutions.
% However, these approaches require a large-scale sampling before ranking, which is impractical for many users due to the high cost.
% However, the large-scale sampling procedure entails high cost and is impractical for many users. 
% \zkc{need edit}
% Inspired by the problem-solving process of human programmers, we propose a generate-and-edit framework that utilizes execution results on the example test case to improve the quality of generated codes by LLMs. Our fault-aware code editors are trained to fix the potential errors in the generated codes with the guidance of any error messages.
% example test case of the problem
% 这句话太长难了，而且附属的内容太多了
Inspired by the problem-solving process of human programmers, we propose a generate-and-edit approach that utilizes test results of the generated code from LLMs to improve the performance of LLMs on the competitive programming task. We execute the generated code on the example test case provided in the problem description and wrap the test results into a supplementary comment for editing. We then design a fault-aware code editor, trained to fix the potential errors in the generated codes with the guidance of the comment.
% In conclusion, our generate-and-edit framework for LLMs provides a promising approach for generating high-quality code for competitive programming tasks. By leveraging the power of LLMs and incorporating human-like problem-solving strategies, our framework enables LLMs to generate code that is more accurate and efficient than previously possible. Our fault-aware neural code editor, which takes the generated code and error messages as input, is key to achieving these improvements. Our experiments show that our approach outperforms other post-processing methods for code generation. As LLMs continue to evolve and become more scalable, developing effective approaches for interacting with these models will be a crucial area of future investigation. We believe it has the potential to advances the field of code generation using LLMs and opens up new possibilities for the development of intelligent systems.
% Our extensive evaluations on two competitive programming datasets and nine different LLMs demonstrate the effectiveness and universality. Compared with directly generating from LLMs, our framework can improve pass@1 by an average of 478\% on APPS-dev , 139\% on APPS-test and 113\% on HumanEval for nine popular code generation LLMs with parameter sizes ranging from 110M to 175B.
Our extensive evaluations of two competitive programming datasets and nine different LLMs demonstrate the effectiveness and universality. Compared with directly generating from LLMs, our approach can improve the average of pass@1 by 89\% on APPS-dev, 31\% on APPS-test, and 48\% on HumanEval over nine popular code generation LLMs with parameter sizes ranging from 110M to 175B.
% 跟谁比说清楚，提升的base是什么
% Even for the chosen largest language model GPT3-175B, our editor model can improve pass@1 from 26.6\%  to 32.4\% on the APPS-dev benchmark.
% \lz{Improve xx\%}
% We also find that editing the code generated by PyCodeGPT (110M) produces comparable results to the GPT-J (6B) model.
In comparison to existing state-of-the-art post-processing methods, our method demonstrates both superior accuracy and efficiency, especially with a limited sample budget.
\end{abstract}

==> section/model.tex <==
\input{table/fig_pipeline.tex}
We now describe our generate-and-edit framework for code generation task. Figure \ref{fig:pipeline} provides an overview of the pipeline procedure. 

The proposed framework for code generation tasks uses large language models as black-box generators, treating them as fixed models that cannot be modified. This design choice is motivated by the fact that training LLMs is costly and access to LLMs is often restricted. ({\textit{E}.\textit{g}.}, OpenAI only offers API access to fine-tune or infer GPT3.) Using LLM as a black-box generator makes our framework flexible for using different LLMs.
% access to these large models is often restricted, and their constant evolution and improvement make treating them as black-boxes a convenient and efficient way to incorporate their capabilities into the framework 
After we generate the programs using the LLM, we run the example test cases with an executor to obtain execution results possibly accompanied with error messages.
Based on the test results, we construct the supplementary comments that provides execution results with error messages for the fault-aware code editor model. The editor is used to refine the code based on the natural language description, generated code, and supplementary comments.

In this framework, we leverage the strengths of large language models and refine the code to address potential errors.

\subsection{LLMs as black-box}

\label{sec:LLM}
The proposed framework uses large language models as fixed generators that cannot be modified. This decision is based on the difficulty of accessing and running these models, as well as the convenience of using them as plug-and-play components that are constantly improving with new generation models. Our approach requires the same number of samples from LLMs as the last number of submissions, which is greatly reduced compared to existing post-processing techniques. Detailed comparision is described in Section \ref{sec:ranking_rst}.
% In this paper, we investigate the effectiveness of several widely used language models for code generation, including \textit{GPT3-davinci-002} (175B) \cite{gpt3}, \textit{CodeGen} (350M, 2B) \cite{codegen}, \textit{InCoder} (1B) \cite{incoder}, \textit{GPT-Neo} (125M, 1.3B) \cite{gpt-neo}, \textit{GPT-J} (6B) \cite{gpt-j} and \textit{PycodeGPT} (110M) \cite{CERT}. These models are evaluated under zero-shot or finetune experimental conditions, with additional descriptions provided as a part of Table \ref{tab:apps_dev}.
% In this paper, we investigate the effectiveness of nine widely used language models for code generation with parameter sizes ranging from 110M to 175B. These models are evaluated under zero-shot or finetune experimental conditions. Additional descriptions are provided as a part of Table \ref{tab:apps_dev}.

% By treating the large language models as black-boxes, we are able to incorporate their capabilities into our framework without the need for extensive expertise or resources.

% In this paper, we study several commonly used families of large language models for code generation, including \ding{172} GPT3 (davinci-002 175B) \footnote{We did not choose the CodeX model designed for programming languages in the GPT3 family, because this model is still in beta and it is difficult to obtain public access.}, \ding{173} CodeGen (350M, 2B), \ding{174} Incoder (1B), \ding{175} GPT-Neo (125M, 1.3B), \ding{176} PycodeGPT(110M). For these models, our experimental settings include zero-shot and finetune experimental settings. The detailed model introduction is shown in the table \zkc{add a table like Fault-Aware Neural Code Rankers}. While our approach is applicable to any of these models, in this study, we validate the effectiveness of our framework on a set of state-of-the-art code generation models that are publicly available and we finetune some models within our computing power on APPS dataset , for reproducibility.

% In this study, we investigate the use of several popular families of large language models for code generation, including GPT3 (davinci-002 175B), CodeGen (350M, 2B), Incoder (1B), GPT-Neo (125M, 1.3B), and PycodeGPT (110M). We conduct experiments using both zero-shot and finetuned settings, and present a detailed model introduction in Table 1. Although our approach is applicable to any of these models, we validate the effectiveness of our framework on a set of state-of-the-art code generation models that are publicly available. Additionally, we finetune some models within our computing constraints on a public competitive programming dataset, APPS, for reproducibility.

% In this paper, we investigate the effectiveness of several widely used language models for code generation, including \textit{GPT3-davinci-002} (175B) \cite{gpt3}, \textit{CodeGen} (350M, 2B) \cite{codegen}, \textit{InCoder} (1B) \cite{incoder}, \textit{GPT-Neo} (125M, 1.3B) \cite{gpt-neo}, \textit{GPT-J} (6B) \cite{gpt-j} and \textit{PycodeGPT} (110M) \cite{CERT}. These models are evaluated under zero-shot or finetune experimental conditions, with additional descriptions provided as a part of Table \ref{tab:apps_dev}. While our approach can be applied to any of these models, in this study we focus on validating its effectiveness on a selection of state-of-the-art code generation models that are publicly available and within the scope of our computing power, and finetunes some of these models on the APPS dataset \cite{APPS} for reproducibility purposes.

\subsection{Executor and Supplementary Comments}
\label{sec:comments}


% 为什么是这三种comment template，这部分应该是技术的核心之一，需要长篇大论一下
After code is generated by the large language model, our framework uses an executor to run on the example test case. We further analyze the execution result and find it can be classified into three types: \ding{182} The generated code pass the example test case. \ding{183} The code executes successfully, but returns incorrect outputs. \ding{184} The code terminate due to an error. By further analyzing the reason for the specific execution result, we find other additional key information for editing: for the case where the incorrect output is returned, the input, output, and expected output of the current code are helpful for rewriting the code. For the case where the code is terminated with an error, including the error type, the description of the error message, the line number where the error occurred, and the specific line content is helpful for fixing potential bugs. Therefore, it is necessary to use some templates to wrap these execution results as a guide for editing.

\input{table/fig_commentexample.tex}
In our approach, for each execution scenario we provide supplementary comments to explain the specific execution situation. Figure \ref{fig:commentexample} shows three different supplementary comment template examples. If the code passes the example test case, we use \textit{Comment 1}. If the code produces incorrect output, we use \textit{Comment 2} and provide the relevant input and output. If the code terminates with an error, we use \textit{Comment 3} and include the line number, line context, and full error message to troubleshoot any potential errors. These supplementary comments are intended to provide additional context and clarity for the generated code, and are used to provide guidance to assist in editing the code.



% Python对error message的定义：https://docs.python.org/3.10/library/exceptions.html?highlight=syntaxerror#SyntaxError
% After code is generated by the large language model, our framework uses an executor to run example test cases and obtain potential error messages. This allows us to identify and address potential errors in the generated code. The executor is designed to run the generated code and collect any error messages that may be produced during execution.
% For each execution scenario, we provide supplementary comments to explain the specific execution situation. Figure \ref{fig:commentexample} shows three different supplementary comment template examples. If the code passes the example test case, we use \textit{Comment 1}. If the code produces incorrect output, we use \textit{Comment 2} and provide the relevant input and output. If the code terminates with an error, we use \textit{Comment 3} and include the line number, line context, and full error message to troubleshoot any potential errors. These supplementary comments are intended to provide additional context and clarity for the generated code, and are used to provide guidance to assist in editing the code.


% \zkc{add a table to describe the supplementary in different situations}
\input{table/fig_comment_distribution.tex}
We observe that the generated programs produced by various language modeling models exhibit distinct styles, as evident in the varying distributions of supplementary comments.  Figure \ref{fig:comment_distribution} shows the distributions for various situations and error classes of the supplementary comments on APPS-train dataset using \textit{PyCodeGPT-110M-finetuned} and \textit{GPT3} models. It is noted that smaller pretrained models, such as \textit{PyCodeGPT-110M-finetuned}, tend to encounter SyntaxError issues more frequently. Conversely, larger models show a decrease in the number of program terminations due to errors, with the handling of wrong outputs becoming a primary focus for the editor.

==> section/preliminaries.tex <==
\subsection{Code Generation}


\subsection{Code Edit}

==> section/relatedwork.tex <==
\subsection{Large Language Models for Code Generation}



\subsection{Post-process for Code Generation models}



\subsection{Automatic Post-editing for LLMs}



==> table/apps_test_difficulty_level.tex <==
\begin{table}[t]
% \footnotesize
    % \setlength\tabcolsep{3pt}
    % \renewcommand\arraystretch{0.8}
    \centering
    \caption{Results on the APPS test dataset with 3 difficulty levels. We use the \textit{Incoder-1B-finetuned} as the base model. For each difficulty level, we show the base model results (the first row) and edited results (shaded row below). The numbers in red indicate the absolute improvements of our editor.}
\centering
\small
\begin{tabular}{clll}
\toprule
% \multicolumn{4}{c}{Base Model: Incoder-1B-finetune}                                                                                           \\
% \midrule
\multicolumn{1}{l}{Difficulty level} & pass@1                       & pass@5                       & pass@10                      \\
\midrule
                                     & 1.60                         & 2.80                         & 3.50                         \\
\multirow{-2}{*}{Introductory}       & \cellcolor[HTML]{F2F2F2}1.80 \increase{0.20}  & \cellcolor[HTML]{F2F2F2}3.30 \increase{0.50} & \cellcolor[HTML]{F2F2F2}4.20 \increase{0.70} \\
\midrule
                                     & 0.53                         & 0.93                         & 1.03                         \\
\multirow{-2}{*}{Interview}          & \cellcolor[HTML]{F2F2F2}0.80 \increase{0.27}  & \cellcolor[HTML]{F2F2F2}1.43 \increase{0.50} & \cellcolor[HTML]{F2F2F2}1.83 \increase{0.80} \\
\midrule
                                     & 0.10                         & 0.30                         & 0.60                         \\
\multirow{-2}{*}{Competition}        & \cellcolor[HTML]{F2F2F2}0.10  & \cellcolor[HTML]{F2F2F2}0.50 \increase{0.20} & \cellcolor[HTML]{F2F2F2}0.80 
 \increase{0.20} \\
\midrule
                                     & 0.66                         & 1.18                         & 1.44                         \\
\multirow{-2}{*}{Average}            & \cellcolor[HTML]{F2F2F2}0.86 \increase{0.20} & \cellcolor[HTML]{F2F2F2}1.62 \increase{0.44} & \cellcolor[HTML]{F2F2F2}2.10 \increase{0.66} \\
\bottomrule
\end{tabular}
\vspace{-2mm}
   \label{tab:apps_test_difficulty}
\end{table}

==> table/apps_test_difficulty_levels_v1.tex <==
\begin{table}[t]
% \footnotesize
    % \setlength\tabcolsep{3pt}
    % \renewcommand\arraystretch{0.8}
    \centering
    \caption{Results on the APPS test dataset with the difficulty levels. We use the \textit{Incoder-1B-finetune} as the base model.}
\centering
\begin{tabular}{ccccc}
\toprule
\multicolumn{5}{c}{Incoder-1B-finetune}                                                                                                                  \\
\midrule
\multicolumn{1}{l}{Difficulty level} & \multicolumn{1}{l}{} & pass@1                       & @5                       & @10                      \\
\midrule
                                     & origin               & 1.60                         & 2.80                         & 3.50                         \\
\multirow{-2}{*}{introductory}       & edit                 & \cellcolor[HTML]{F2F2F2}1.8  & \cellcolor[HTML]{F2F2F2}3.30 & \cellcolor[HTML]{F2F2F2}4.20 \\
                                     & origin               & 0.53                         & 0.93                         & 1.03                         \\
\multirow{-2}{*}{interview}          & edit                 & \cellcolor[HTML]{F2F2F2}0.8  & \cellcolor[HTML]{F2F2F2}1.43 & \cellcolor[HTML]{F2F2F2}1.83 \\
                                     & origin               & 0.10                         & 0.30                         & 0.60                         \\
\multirow{-2}{*}{competition}        & edit                 & \cellcolor[HTML]{F2F2F2}0.1  & \cellcolor[HTML]{F2F2F2}0.50 & \cellcolor[HTML]{F2F2F2}0.80 \\
\midrule
                                     & origin               & 0.66                         & 1.18                         & 1.44                         \\
\multirow{-2}{*}{average}            & edit                 & \cellcolor[HTML]{F2F2F2}0.86 & \cellcolor[HTML]{F2F2F2}1.62 & \cellcolor[HTML]{F2F2F2}2.10 \\
\bottomrule
\end{tabular}
\vspace{-2mm}
   \label{tab:apps_test_difficulty_v1}
\end{table}

==> table/comments.tex <==
\begin{table}[t]
% \footnotesize
    \setlength\tabcolsep{5pt}
    % \renewcommand\arraystretch{0.8}
    \centering
    \caption{Examples of the supplementary comments, TODO}
\centering
\begin{threeparttable}
\begin{tabular}{lccccc}
\toprule
Model       & Java250 & Python800 & C++1000        & C++1400        & POJ-104 \\ \midrule
RGCN        & 91.93   & 91.60      & 92.73          & 92.34          & 95.57   \\
GGNN        & 93.64   & 92.23     & 91.72          & 92.48          & 94.80    \\ \midrule
TBCNN       & 92.84   & 93.17     & 94.77          & 88.29          & 96.20    \\
ASTNN       & 92.86   & 93.80     & 94.61          & 90.17          & 96.79     \\
TreeCaps    & 93.07   & 94.35     & 94.92          & 90.16          & 96.81   \\ \midrule
SBT         & 65.64   & 71.69     & 65.05          & 56.33          & 89.58   \\
X-SBT       & 83.31   & 89.10      & 66.79          & 67.00          & 94.58   \\ \midrule
Transformer & 93.49   & 93.99     & 89.93          & 67.87          & 88.13  \\
GREAT       & 93.36   &  93.27      & 92.76          & 92.50          & 90.33  \\ \midrule
\textbf{HiT}         & \textbf{94.81}   & \textbf{95.97}     & \textbf{95.05} & \textbf{93.27} & \textbf{97.08}   \\ \midrule
% C-BERT       & 97.40   & 97.09      & 93.79          &  91.83          & -  \\ 
\textit{CodeBERT}\tnote{$\dagger$}       & \textbf{\textit{96.47}}   &  \textbf{\textit{97.41}}      & \textit{86.13}           &  \textit{83.05}          & \textbf{\textit{98.40}}  \\ 
\bottomrule
\end{tabular}
\begin{tablenotes}
\footnotesize
     \item[$\dagger$] CodeBERT is a pre-trained model with significantly more parameters than our model, with a parameter count nearly 27 times that of HiT.
\end{tablenotes}
   \label{tab:res_cls}
\end{threeparttable}

\end{table}

==> table/compared_rerank.tex <==
\begin{table}[t]
% \footnotesize
    % \setlength\tabcolsep{3pt}
    % \renewcommand\arraystretch{0.8}
    \centering
    \caption{Pass Rate Results compared with a state-of-the-art reranking methods on the APPS dataset. We copy the results reported by the corresponding paper here and reproduce their baseline results with our editors. We use the \textit{GPT-Neo-1.3B-finetuned} as the base model.}
\centering
% \small
\scriptsize
\begin{tabular}{crccccc}
\toprule
% \multicolumn{6}{c}{GPT-Neo-1.3B-finetune}                                                                          \\
% \midrule
\multicolumn{1}{l}{}         &    &          & \multicolumn{2}{c}{APPS-dev}  & \multicolumn{2}{c}{APPS-test} \\
\midrule
\multicolumn{1}{l}{}         & {\scriptsize Setting}  & {\scriptsize Samples}    & @1        & @5        & @1        & @5        \\
\midrule
\multirow{2}{*}{\scriptsize \begin{tabular}[c]{@{}c@{}}Reported in\\ \cite{inala2022faultaware}\end{tabular}}     & {\tiny base model} & 100   & 2.6           & 9.1           & 0.14          & 0.53          \\
                             & {\tiny + ranker} & 100 & 8.0             & 15.1          & 0.3           & 1.1           \\
\midrule
\multirow{2}{*}{\scriptsize {Our results}} & {\tiny base model} & \{1,5\}   & 4.0             & 10.9          & 0.14          & 0.74          \\
                             & {\tiny + editor} & \{1,5\} & \textbf{10.5} & \textbf{18.6} & \textbf{0.68} & \textbf{1.38} \\
\bottomrule
\end{tabular}
\vspace{-2mm}
   \label{tab:compared_rerank}
\end{table}

==> table/diffeditor.tex <==
\begin{table}[t]
% \footnotesize
    % \setlength\tabcolsep{3pt}
    % \renewcommand\arraystretch{0.8}
    \centering
    \caption{Results of different editors on APPS-dev using \textit{PyCodeGPT} and \textit{GPT3} as base models.}
\centering
\small
\begin{tabular}{cccc}
\toprule
\multicolumn{1}{l}{}           &                         & \multicolumn{2}{c}{APPS-dev}        \\
\midrule
\multicolumn{1}{l}{Base Model} & Editor                  & pass@1               & pass@5       \\
\midrule
\multirow{4}{*}{PyCodeGPT}     & base model              &                      &              \\
                               & \othereditor{PyCodeGPT}        &                      &              \\
                               &  \othereditor{InCoder}       &                     &              \\
                               & \othereditor{GPT3}             &                      &              \\
\midrule
\multirow{3}{*}{GPT3}          & base model              &                      &              \\
                               & \othereditor{GPT3}             &                      &              \\
                               & \othereditor{PyCodeGPT}        &                      &             \\
\bottomrule
\end{tabular}
\vspace{-2mm}
   \label{tab:diffedit}
\end{table}
